CSM-NN: Current Source Model Based Logic Circuit Simulation -- A Neural Network Approach

The miniaturization of transistors down to 5nm and beyond, plus the increasing complexity of integrated circuits, significantly aggravate short channel effects, and demand analysis and optimization of more design corners and modes. Simulators need to model output variables related to circuit timing, power, noise, etc., which exhibit nonlinear behavior. The existing simulation and sign-off tools, based on a combination of closed-form expressions and lookup tables are either inaccurate or slow, when dealing with circuits with more than billions of transistors. In this work, we present CSM-NN, a scalable simulation framework with optimized neural network structures and processing algorithms. CSM-NN is aimed at optimizing the simulation time by accounting for the latency of the required memory query and computation, given the underlying CPU and GPU parallel processing capabilities. Experimental results show that CSM-NN reduces the simulation time by up to $6\times$ compared to a state-of-the-art current source model based simulator running on a CPU. This speedup improves by up to $15\times$ when running on a GPU. CSM-NN also provides high accuracy levels, with less than $2\%$ error, compared to HSPICE.

==> experiment.tex <==


\section{Experiments and Simulation Results} \label{sec:experiments}

We implemented the simulator and the flow of our CSM-NN framework in Python. Our implementation 
is technology independent and can characterize, and create NN models with flexible configurable setup, for any given combinational circuit netlist. NN implementation and training are based on the Scikit-learn~\cite{scikit-learn} package. 

CPU and GPU devices introduced in Table~\ref{tab:cpu-spec} and Table~\ref{tab:gpu-spec} are used for comparison between two platforms, as both products are introduced in the same year (2016) and their current retail prices are in the same order (of about 5,000 USD). 
In this following, we discuss our experiments including challenges regarding our specific problem setup. 

\subsection{Selected Technologies}
 In this work, for better evaluation of our CSM-NN including its technology independent characteristics, we performed our experiments on both MOSFET (16nm) and FinFET (20nm) device technologies from Predictive Technology Model~(PTM)~\cite{PTM} packages. Two device types namely \textit{low-standby power} (LP) and \textit{high performance} (HP) are used in our experiments~\cite{finfet-msa}.

% I added my own paper here lol
%For the case of deeply scaled devices, the optimal choice of devices characteristics  has a significant impact on energy and timing efficiencies for different applications and modes~\cite{finfet-msa}. 
%Our experimental results in the following include defined in each technology. 

As technology scales down, a growing number of physical and fitting parameters are needed to model PVT variations.
%This is not only limited to parameters representing real physical features, but also includes fitting parameters. 
However as pointed out in~\cite{TED2016-UCB, Dadgour-ICCAD2008,Matsukawa-2009, IEDM2009-Stanford-SRAM}, only a few of them are dominant, i.e., developing simulation models that account for those dominant parameters while ignoring the rest, provides sufficiently high accuracy levels. 
% One benefit of ML is that identification of those dominant parameters can be done systematically. 
Following these studies, we considered the most important process variation factors for defining a limited number of process corners. % Our experiments confirm that metal gate work function ($\Phi_M$), channel doping ($N_A$), and thickness of oxide ($t_{ox}$) and Fin ($t_{fin}$) are dominant. 
There is no process variation distribution information available for PTM technologies. 
Therefore, we followed the same approach used in~\cite{PV-MOSFET-2010} which studied the same devices as this work to define PVT corners. 

All distributions but temperature are considered normal (Gaussian) and reported as $N(\mu, \sigma)$ with ($\mu$) and ($\sigma$), representing mean and standard deviation respectively. The typical temperature value is considered as 27\textdegree{C} and the highest temperature ($+3\sigma$ variation) as 125\textdegree{C}. 
The information of the distribution for process variation parameters and the defined process corners for experiments are provided in Table~\ref{tab:ptm-pvt}. 

\vskip 3mm
\begin{table}[h]
\caption {Process (P), Voltage (V), and Temperature (T) variation distributions of technologies used in experiments. The values of process attributes are reported for NMOS/NFET devices. $t$ is representing \textit{oxide thickness} ($t_{ox}$) for MOSFET and \textit{Fin thickness} ($t_{fin}$) for FinFET. The distributions are all Normal($\mu, \sigma$) and represented as ($\mu, \sigma$).} \label{tab:ptm-pvt}
\centering
\begin{tabular}{l|l|l|l|l|l}
\multicolumn{1}{c}{} & \multicolumn{5}{c}{PVT Variation Distribution} \\ \hline \hline
\multicolumn{2}{l|}{Technology}  & $V_{dd} (v)$  &   $\Phi_M (ev)} & $N_A (1e20)$ & $t (nm)$ \\  \hline
\multicolumn{2}{l|}{Fin-LP} & 0.9,0.05    & 4.6,0.23    & -      & 15,0.5 \\
\multicolumn{2}{l|}{Fin-HP} & 0.9,0.05    & 4.4,0.22    & -      & 15,0.5 \\ 
\multicolumn{2}{l|}{MOS-LP} & 0.9,0.05    & 4.6,0.23    & 2,0.1  & 1.2,0.04 \\ 
\multicolumn{2}{l|}{MOS-HP} & 0.7,0.035   & 4.4,0.23    & 2,0.1  & 0.95,0.03 \\ 
\multicolumn{6}{c}{} \\ 
\end{tabular}
\begin{tabular}{l|l|l|l|l|l}
\multicolumn{1}{c}{} & \multicolumn{5}{c}{PVT variation in pre-defined corners} \\ \hline \hline
Corner & $V_{dd}(v)$ & $T$(\textdegree{C}) & $\Phi_M (ev)$ & $N_A$ & $t(nm)$ \\ \hline
FF   & $+3\sigma$ & $0\sigma$ & $-3\sigma$ & $+3\sigma$ & $-3\sigma$ \\ 
SS   & $-3\sigma$ & $0\sigma$ & $+3\sigma$ & $-3\sigma$ & $+3\sigma$ \\ 
FFHT & $+3\sigma$ & $+3\sigma$ & $-3\sigma$ & $+3\sigma$ & $-3\sigma$ \\ 
SSHT & $-3\sigma$ & $+3\sigma$ & $+3\sigma$ & $-3\sigma$ & $+3\sigma$ \\ 
\end{tabular}
\end{table}

\vskip 5mm

\subsection{Characterization}
The resolution of characterization process is a key factor in determining the accuracy of both CSM-LUT and CSM-NN simulations. 
While more data points increase the accuracy of both simulators, it comes with the cost of longer characterization process, larger tables in CSM-LUT, and longer training time in our CSM-NN. 
We therefore evaluate our CSM-NN framework under different resolutions. The results can also be later used towards suggesting a baseline for other technologies. 
%The resolution of characterization process is a key factor in determining the accuracy of both CSM-LUT and CSM-NN simulations. 
% While choosing more data points increases the accuracy of both simulators, it also requires longer characterization time, larger tables in CSM-LUT and longer training time in CSM-NN. 

It should be mentioned that CSM-components exhibit different sensitivity levels to different voltage-node variables. For example, $C_O$ seems to be more sensitive to $V_O$ than $V_I$ in INVX1, and it can be characterized with lower resolution for $V_I$ than $V_O$. Moreover, the sensitivity to resolution of characterization for one CSM-component should not be necessarily the same as the other component. For example, the range of change in $I_o$ value for a single $INVX1$ transition is from $\mu A$ to $nA$, while this is about only $50\%$ for $C_O$. 
The resolution can also vary based on the range of the voltage-node variable, e.g., higher resolutions for the noisy parts of the waveform (with higher frequencies of change) and lower resolutions for smooth parts of the waveforms.

However, for the sake of simplicity, we considered all voltage-node resolutions as similar.
As the units for different dimensions are different, we defined three different resolution setups as explained in Table~\ref{tab:char-res}. 
By comparing the preliminary results, \textit{normal} setup was found to be an appropriate resolution and the experiments were continued with this setup. 



\begin{table}[!h]
\centering
\caption {Characterization resolution settings used in our experiments.} 
\label{tab:char-res} 
\begin{tabular}{l|c|c|c}
 & S: Soft & N: Normal & C: Coarse \\ \hline
Resolution (v)& 0.01 & 0.05  & 0.1 \\ 
\end{tabular}
\end{table}


\begin{table}
\centering
\caption {Choice of NN hidden layer size for single and two input logic cells.} 
\label{tab:cell-NN} 
\begin{tabular}{l|l|l|l|l|l}
& TT & FF & SS & FFHT & SSHT \\ \hline \hline
\multicolumn{6}{c}{MOSFET-HP 16nm} \\ \hline 
INV & 14 & 16 & 18 & 16 & 18 \\ 
NAND2 & 24 & 28 & 30 & 28 & 30 \\ \hline \hline
%
\multicolumn{6}{c}{MOSFET-LP 16nm} \\ \hline
INV & 20 & 20 & 24 & 22 & 26 \\ 
NAND2 & 28 & 32 & 30 & 32 & 32 \\ \hline \hline
%
\multicolumn{6}{c}{FinFET-HP 20nm} \\ \hline
INV & 20 & 20 & 20 & 26 & 24 \\ 
NAND2 & 34 & 30 & 34 & 36 & 36 \\ \hline \hline
%
\multicolumn{6}{c}{FinFET-LP 20nm} \\ \hline
INV & 20 & 20 & 20 & 26 & 20 \\ 
NAND2 & 30 & 36 & 36 & 40 & 38 \\ \hline \hline
\end{tabular}
\end{table}



\begin{table*}
\centering
\caption{CSM simulation results of a full adder circuit in both FinFET and MOSFET technologies. The simulation time improvements ($A$) is the ratio of the time required for CSM-LUT simulation over the one for CSM-NN. While CSM-LUT results would not improve if they were run on a GPU (instead of a CPU), the improvement results for the CPU and GPU implementation of CSM-NN are reported as $A_{CPU}$ and $A_{GPU}$ respectively. The hardware platform's specs are reported in Table~\ref{tab:cpu-spec} and~\ref{tab:gpu-spec}. $E_{sim}$ is the measure of accuracy introduced in Eq.~\ref{eq:esim}. }
\label{tab:res-FA}
\begin{minipage}{\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
- & \multicolumn{3}{c|}{\textbf{MOSFET-HP 16nm}} & \multicolumn{3}{c|}{\textbf{MOSFET-LP 16nm}} & \multicolumn{3}{c|}{\textbf{FinFET-HP 20nm}} & \multicolumn{3}{c|}{\textbf{FinFET-LP 20nm}} \\ \hline
Corner 	& $E_{sim.}$ & $A_{CPU}$ & $A_{GPU}$ & $E_{sim.}$ & $A_{CPU}$ & $A_{GPU}$ & $E_{sim.}$ & $A_{CPU}$ & $A_{GPU}$ & $E_{sim.}$ & $A_{CPU}$ & $A_{GPU}$ \\ \hline
Nominal & \textless 2\% & 9.3 & 16.8 & \textless 2\% & 9.3 & 16.8 & \textless 2\% & 6.9 & 15.1 & \textless 2\% & 8.6 & 16.8 \\ \hline
FF  	& \textless 2\% & 8.6 & 16.8 & \textless 1\% & 7.4 & 15.1 & \textless 2\% & 8.6 & 16.8 & \textless 2\% & 6.8 & 15.1 \\ \hline
SS      & \textless 2\% & 8.6 & 16.8 & \textless 2\% & 6.9 & 15.1 & \textless 1\% & 6.9 & 15.1 & \textless 1\% & 6.8 & 15.1 \\ \hline
FFHT 	& \textless 2\% & 8.6 & 16.8 & \textless 1\% & 7.4 & 15.1 & \textless 1\% & 6.8 & 15.1 & \textless 2\% & 6.6 & 15.1 \\ \hline
SSHT 	& \textless 2\% & 8.6 & 16.8 & \textless 1\% & 7.4 & 15.1 & \textless 1\% & 6.8 & 15.1 & \textless 1\% & 6.6 & 15.1 \\ \hline
\end{tabular}
\end{minipage}
\end{table*}




\subsection{Preprocessing and Loss Function Modification}
Mean Square Error (MSE, also referred as L2-norm error) is a commonly used regression loss function. It is simply the average of squared distances between our targets ($y_i$) and predicted values ($\hat{y_i}$). The loss function can also accommodate regularization term added to the loss function in order to prevent overfitting by shrinking the model parameters. The values of CSM-components vary in a large scale. For example, in INV, with  $V_{I}$, $V_{O}$ as variables, the DC current $I_{D}$ is in $micro-scale$ when both transistors are on, while in $nano-scale$ when one of them is off and the cell is leaking. 
The MSE-loss is a function of absolute error. Thus, by using this loss, the error in lower scale values will be less important compared to the higher scale values. To address this, we can log-transform the output, so the relative error will be used for loss calculation of the regression model as shown in Eq.\ref{eq:MSE}. An issue with such an adjustment is that some of the values are negative and this makes the log-transform more complicated. We simply resolved such issue with a simple shift of data toward positive values by subtracting all data points with their overall minimum $y_{min}$. 

\begin{equation}
\label{eq:MSE}
\begin{split}
MSE &= \frac{\sum_{i=0}^{N} (y_{i} - \hat{y_i} )^2}{N} \\
MSE_{log} &= \frac{\sum_{i=0}^{N} (log(y_{i}-y_{min}) - log(\hat{y_i} - y_{min}))^2} {N} \\
% &= \frac{\sum_{i=0}^{N} (log \frac{y_{i}}{\hat{y_i}})^2}{N} 
\end{split}
\end{equation}

The normalization of data in regression problems would help the solvers with faster convergence and better numerical stability. Hence, normalization of inputs and outputs is typically implemented inside the solver, such as that in the Scikit-learn package~\cite{scikit-learn}  used in our implementation.




\subsection{NN Size and Training for Logic Cells}
To select the size of the hidden layer for each model, we repeated the training process for various neuron numbers in the range of $10-50$.
Preliminary results in our experiments showed that the \textit{tanh} nonlinear function provides better outcomes compared to other functions such as \textit{sigmoid} and \textit{ReLU}. 
As mentioned in Section~\ref{sec:nn-training}, there is no hyper-parameter, e.g., no learning-rate or mini-batch size tuning is required in L-BFGS optimization. 

The total number of generated data points is 500 per gate. We trained the NN with 90\% of this data (5-fold cross-validation, 360 for training and 40 for validation) and then tested on the other 10\%. The split between training, validation, and test datasets was done in random. 

Next, we applied a few noisy input smaples to the cell and measured $E_{sim}$. 
The minimum size of the hidden layer that met $E_{sim} < 1 \%$ is chosen as the CSM-NN architecture for the logic cell in the specific MCMM setup. 
The complete results for the choice of architecture for INV and NAND2 are given in Table~\ref{tab:cell-NN} for different MCMM setups. 


\subsection{Circuit Simulation}
In this work we evaluated our CSM-NN framework by simulating a full-adder circuit (schematic shown in Fig.~\ref{fig:full-adder}). 

For the sake of a fair comparison, the HSPICE characterization setup is the same for both CSM-NN and CSM-LUT. 
We measured $E_{sim}$ by comparing output waveforms of HSPICE as the baseline with those of CSM-NN simulations. 
 The CPU and GPU devices used in our experiments are introduced in Table~\ref{tab:cpu-spec} and Table~\ref{tab:gpu-spec} respectively. 
CSM-LUT is considered to be computed on the CPU platform as it does not benefit from GPU parallelization. 
The required computation resources and latencies are calculated using equations in section~\ref{sec:neural-network}. 
The results confirm that CSM-NN output waveforms match those of HSPICE in regard to propagation delay with error values limited to 0.1\%. To better confirm the high accuracy of CSM-NN, we compared its waveform similarity to HSPICE, by measuring $E_{sim}$. As listed in Table~\ref{tab:res-FA}, $E_{sim}$ is limited to 2\%.

\begin{figure}
\centering
\includegraphics[width=0.37\textwidth, keepaspectratio] {figures/FA_NAND.pdf}
\caption{Gate level schematic of the full adder circuit used in our experiments.}
\label{fig:full-adder}
\end{figure}



==> variation.tex <==

\section{Process Variation PLEASE DON'T READ} \label{sec:process-variation}

As technology geometries continue to shrink to nano-meter scale, the ability to control critical device parameters is becoming increasingly difficult. This includes the dimensions, doping concentrations, orientation of metal grains and etc. Beside continuous technological improvements in creating new devices with more advanced fabrication processes, the problem of timing analysis under process variation is becoming more challenging and more accurate modeling is inevitable to accomplish timing and yield requirements. 

There are two main categories of process variations: (1) Systematic variation are deterministic in nature and can be attributed to the layout or fabrication equipment related effects. Thus they generally show spatial correlation behaviour in the chip (2) Random or non-systematic variation are unpredictable in nature, such as dimensions of gate/Fin (length, width, oxide thickness), doping fluctuation and even orientation of fabrication particles. Variations of this sort can vary independently for each device on a chip. 

There are other ways of classifying process variation such as intra or inter die, and front or back end variations, which are not the focus of this article. % Do I really need this? 

Manufacturer provides the information of process variation alongside the technology files. The number of parameters with process variation are vast. While most of these parameters are representing real physical features, some are fitting variables and don't have any physical meaning. To make sure the circuit work in different situations, Monte Carlo simulation is done. 

Considering the large number of parameters, the time complexity of Monte Carlo simulation is too much. This is why the status quo is to limit the process variation parameters to the most important ones to be able to do simple (maybe pre-final) simulations. The impact and type of sources are variation are different between technologies. As an example of new fabrication technology, by spacer lithography becoming prevalent for the last few years, the impact of Line Edge Roughness (LER) is not significant source of variation in FinFET devices. Moreover, while random dopant fluctuation (RDF) is a dominant in bulk planar MOSFET devices, it's impact does not exist in undoped FinFET devices. Replacing polysilicon with metal-gate resolved the various difficulties of using high-K materials and increased the $I_{ON}$ current of the devices. However, the metal work function is very dependent on the orientation of metal grains which is not controllable during the growth period and is then random. With the scaling of the gate area, it is expected to have about (\textasciitilde 10 \textasciitilde 100) of grains and this will add up to the variation scale of this parameter~\cite{Dadgour-ICCAD2008}.

Different experimental \cite{TED2016-UCB}, \cite{Matsukawa-2009} and analytical \cite{IEDM2009-Stanford-SRAM}, \cite{Dadgour-ICCAD2008} investigated the impact of process variation elements and compared bulk planar MOSFETs and FinFETs in different technology sizes. While the FinFET devices show less variation due their undoped channels and absence of RDF, the main element of variation will be WFV, which will dramatically increase as the sizes are scaled down as described earlier. In this work we refer to these works and consider the parameters of variation as shown in Fig.~\ref{fig:PV-elements}.

\begin{figure}[]
  \centering
  \subfloat[Redrawn from xXx]{\includegraphics[width=0.4\textwidth]{figures/Dadgour-Fig8.png}\label{fig:f1}}
  \hfill
  \subfloat[Redrawn from yYy]{\includegraphics[width=0.4\textwidth]{figures/Matsukawa-Fig13.png}\label{fig:f2}}
  \caption{(a) Comparison between different sources of random variation for a bulk device. (b) Total random Vth  variation for bulk, FD-SOI and FinFET devices in different technology nodes. The metal material is considered to be TiN for both cases. (c) Linear and saturation Vt variations with their sources for 20-nm-Lg (LSTP) bulk planar MOSFET and FinFET predicted by TCAD considering the smallest AVt for MG FinFET and its increase with scaling LW.} 
  \label{fig:PV-elements}
\end{figure}


% \textbf{How is it handled in CSM:} 
In order to handle process variation, authors in \cite{CSM2} store the CSM lookup tables under the nominal process conditions, and apply polynomial corrections for process variations. The first-order method presented in this paper can provide high accuracy for CMOS devices operating in super-threshold regime. However, for FinFET devices operating in the sub/near-threshold regime, the relationship between the driving current and the gate voltages (and the threshold voltage) becomes exponential. Hence, the polynomial correction method is not sufficient to capture the process variations for FinFET devices operating in the sub/near-threshold regime. To solve this problem, authors in \cite{CSM3} introduce a semi-analytical method which stores the pre-characterized regression coefficients in separate lookup tables.

% \textbf{Why should we consider it? }
% \textbf{How is it handled in STA? }
% \textbf{Why current approaches for handling the process variation are not good?} Just a few lines right now that the reader is fresh about how current methods are not working. 


% Process Variation Resources:
% https://www.design-reuse.com/articles/41330/cmos-soi-finfet-technology-review-paper.html
% GIDL in Doped and Undoped FinFET Devices for Low-Leakage Applications
% Variability Analysis of FinFET-Based Devices and Circuits Considering Electrical Confinement and Width Quantization 
% ITRS 2007 report: https://www.semiconductors.org/resources/2007-international-technology-roadmap-for-semiconductors-itrs/
% ITRS 2007 variation maybe is here: https://www.semiconductors.org/wp-content/uploads/2018/08/2007FEP.pdf
% Tunnel-FET Transistors for 13nm Gate-Length and Beyond
% Investigation and Simulation of Work-Function Variation for III–V Broken-Gap Heterojunction Tunnel FET
% Good article online: http://asic-soc.blogspot.com/2008/03/process-variations-and-static-timing.html

